Ludics without Designs I: Triads

In this paper, we introduce the concept of triad. Using this notion, we study, revisit, discover and rediscover some basic properties of ludics from a very general point of view.

==> eptcsdata.tex <==
\providecommand{\firstpage}{49}
\providecommand{\publicationstatus}{S. Alves and I. Cervesato (Eds): Third International Workshop\\ on Linearity 2014 (LINEARITY'14)\\
EPTCS 176, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.176.5}{10.4204/EPTCS.176.5}}
\pdfoutput=1

